Green's function in general relativity

This report provides Green's functions (classical propagators) of gravitational fields appearing in general relativity. The existence of Green's function of the wave equation in curved space with an indefinite metric is ensured owing to the Hodge harmonic analysis. The analyticity of Green's function is determined intrinsically to keep a causality. This report proposed a novel definition of momentum space in curved space-time and the linearisation of the Einstein equation as a free field consistent with that of the Yang-Mills gauge field. The proposed linearisation does not utilize the weak-field approximation; thus, the method applies to highly caved space-time. We gave two examples of Green's function of gravitational fields: the plane wave solution and the Schwarzschild solution.

==> back-up-1.tex <==
\koko{kokokara}
Suppose $\HHH$ is a harmonic form in the amphometric space fulfiling $\Delta_\theta\HHH=0$.
We set component representations of $d\bm\HHH$ and $\cod\bm\HHH$, respectively,  as
\begin{subequations}
\begin{align}
\Omega^{p+1}(\TsMg){\ni}d\bm\HHH&:=H^{~}_{i_{1:p+1}}(\theta)\eee^{i_{1:p+1}},\label{Hcomp1}\\
\Omega^{p-1}(\TsMg){\ni}\cod\bm\HHH&:=\bar{H}^{~}_{i_{1:p-1}}(\theta)\eee^{i_{1:p-1}},\label{Hcomp2}
\end{align}
where $H^{~}_{\bullet},\bar{H}^{~}_{\bullet}\in\R$. 
\end{subequations}
Differential and co-differential operators in the amphimetric space depend on the parameter $\theta$; thus, their tensor coefficients also depend on $\theta$.
We assume the coefficient functions are smooth concerning $\theta$.

%
% Remark
%
\begin{remark}\label{rem6}
Suppose $\HHH\in\Omega^p(\TsMg)$ is the harmonic $p$-form and its $($co-$)$differential have component representations \textup{(\ref{Hcomp1})} and \textup{(\ref{Hcomp2})}.
When $d\bm\HHH$ and $\cod\bm\HHH$ fulfil
\begin{align}
\left\{
\begin{array}{rlclclclclcl}
~&(\sum\bar{H}^{2}_{0i_{1:p-2}}(\pm1/2)&\hspace{-1em}\neq\hspace{-1em}&\sum{H}^{2}_{0i_{1:p}}(\pm1/2)&\hspace{-1em}\Lor\hspace{-1em}&
     \sum\bar{H}^{2}_{j_{1:p-1}}(\pm1/2)&\hspace{-1em}\neq\hspace{-1em}&0&\hspace{-1em}\Lor\hspace{-1em}&
     \sum H^{2}_{j_{1:p+1}}(\pm1/2)&\hspace{-1em}\neq\hspace{-1em}&\left.0\)\\
%%
 \!\Land\hspace{-1em}
 &( \sum\bar{H}^{2}_{j_{1:p-1}}(\pm1/2)&\hspace{-1em}\neq\hspace{-1em}&\sum{H}^{2}_{j_{1:p+1}}(\pm1/2)&\hspace{-1em}\Lor\hspace{-1em}&
       \sum\bar{H}^{2}_{0i_{1:p-2}}(\pm1/2)&\hspace{-1em}\neq\hspace{-1em}&0 &\hspace{-1em}\Lor\hspace{-1em}&
       \sum H^{2}_{0i_{1:p}}(\pm1/2)&\hspace{-1em}\neq\hspace{-1em}&0)\\
 %%
 \!\Land\hspace{-1em} 
 &( \sum\bar{H}^{2}_{0i_{1:p-2}}(\pm1/3)&\hspace{-1em}\neq\hspace{-1em}&\sum H^{2}_{j_{1:p+1}}(\pm1/3)&\hspace{-1em}\Lor\hspace{-1em}&
        \sum\bar{H}^{2}_{j_{1:p-1}}(\pm1/3)&\hspace{-1em}\neq\hspace{-1em}&0&\hspace{-1em}\Lor\hspace{-1em}& 
        \sum{H}^{2}_{0i_{1:p}}(\pm1/3)&\hspace{-1em}\neq\hspace{-1em}&0)\\
%%
\!\Land\hspace{-1em}
&( \sum\bar{H}^{2}_{0i_{1:p-2}}(\pm1)&\hspace{-1em}\neq\hspace{-1em}&\sum H^{2}_{j_{1:p+1}}(\pm1)&\hspace{-1em}\Lor\hspace{-1em}&
       \sum\bar{H}^{2}_{j_{1:p-1}}(\pm1)&\hspace{-1em}\neq\hspace{-1em}&0&\hspace{-1em}\Lor\hspace{-1em}& 
       \sum{H}^{2}_{0i_{1:p}}(\pm1)&\hspace{-1em}\neq\hspace{-1em}&0)\\
%%
\!\Land\hspace{-1em}
&( \sum\bar{H}^{2}_{j_{1:p-1}}(\pm1)&\hspace{-1em}\neq\hspace{-1em}&\sum{H}^{2}_{0i_{1:p}}(\pm1)&\hspace{-1em}\Lor\hspace{-1em}&
       \sum\bar{H}^{2}_{0i_{1:p-2}}(\pm1)&\hspace{-1em}\neq\hspace{-1em}&0&\hspace{-1em}\Lor\hspace{-1em}& 
       \sum H^{2}_{j_{1:p+1}}(\pm1)&\hspace{-1em}\neq\hspace{-1em}&0)
\end{array}\right.,
\label{Hconds}
\end{align}
we obtain
\begin{align}
\Delta_\theta\bm\HHH=0\iff
d\bm\HHH=\cod\bm\HHH=0.\label{dHzero}
\end{align}
for $\theta\in[-1,1]$.\QED
\end{remark}Owing to the assumption, $u(x,\theta)$ and $f(x,\theta)$ are smooth functions concerning the parameter $\theta$. 
Thus, we have the Taylor expansion on a standard basis.
When (\ref{apriori}) is still true at $\theta=\theta_0+\delta_\theta$, we can manipulate the equation as

\begin{proof}
The harmonic form yields
\begin{align}
%~^{\forall}\theta\in(-1,1),\quad
0&=\<\bm\HHH|\Delta_\theta\bm\HHH\>\simeq
\<d\bm\HHH\>^2+\<\cod\bm\HHH\>^2.\label{dHdH0}
\end{align}
We show the (co-)differential pre-norm squared using their coefficients as
%\begin{widetext}
\begin{align*}
&\<d\bm\HHH\>^2=
e^{i\pi p\hspace{.1em}\theta}\sum_{i_1<{\cdots}<i_p}\hspace{-.3em}\(H^{~}_{0i_{1:p}}(\theta)\)^2+
e^{i\pi (p+1)\theta}\sum_{j_1<{\cdots}<j_{p+1}}\hspace{-.3em}\(H^{~}_{j_{1:p+1}}(\theta)\)^2\!,\\
%
&\<\cod\bm\HHH\>^2=
e^{i\pi(p-2)\theta}\sum_{i_1<{\cdots}<i_{p-2}}\hspace{-.4em}\(\bar{H}^{~}_{0i_{1:p-2}}(\theta)\)^2+
e^{i\pi(p-1)\theta}\sum_{j_1<{\cdots}<j_{p-1}}\hspace{-.4em}\(\bar{H}^{~}_{j_{1:p-1}}(\theta)\)^2\!,
\end{align*}
where $\sum H_\bullet^2,\sum \bar{H}_\bullet^2>0$.
Here, we write spatial coefficients separately from coefficients including a zeroth  (time) component.
We obtain that
\begin{align*}
&\<d\bm\HHH\>^2+\<\cod\bm\HHH\>^2=e^{i\pi(p-2)\theta}\(
                        \sum\bar{H}^{2}_{0i_{1:p-2}}(\theta)+
e^{i\pi\theta}\sum\bar{H}^{2}_{j_{1:p-1}}(\theta)+
e^{2i\pi\theta}\sum H^{2}_{0i_{1:p}}(\theta)+
e^{3i\pi\theta}\sum H^{2}_{j_{1:p+1}}(\theta)
\)\!,
\end{align*}
%\end{widetext}
Monomials $A_m\hspace{.1em}e^{i\pi\hspace{.1em}\theta m}$, with $A_m\!\in\!\R$ and $m\!=\!0,1,2,3$, are linearly independent in $\theta\!\in\!(-1,1)\!\setminus\!\{\pm1/2,\pm1/3\}$.
In reality, we obtain that
\begin{align}
\theta=\pm1\hspace{.9em}&\implies
\{e^{0i\pi\theta},e^{1i\pi\theta},e^{2i\pi\theta},e^{3i\pi\theta}\}=\{+1,-1,+1,-1\},\notag\\
\theta=\pm1/2&\implies
\{e^{0i\pi\theta},e^{1i\pi\theta},e^{2i\pi\theta},e^{3i\pi\theta}\}=\{+1,+i,-1,-i\},\notag\\
\theta=\pm1/3&\implies
\{e^{0i\pi\theta},e^{3i\pi\theta}\}=\{+1,-1\},\notag\\
%
\intertext{yielding}
%
\text{(\ref{Hconds})}\Land\text{(\ref{dHdH0})}&\implies
\(\<d\bm\HHH\>=0\Land\<\cod\bm\HHH\>=0\)\overset{\bf{Lemma}~\text{\ref{regularity}}}{\implies}
\text{(\ref{dHzero})}.\label{dHdH2}
\end{align}
Therefore, the remark is maintained.
\end{proof}
\koko{kokomade $\uparrow$}

\koko{koko $\downarrow$}
We can extend a region in which the solution exists from $\theta=0$ toward $\theta=1$ during $\|u(x,\theta)\|^{~}_{L^2}<\infty$.
Since $u(x,\theta)$ is a smooth function concerning $\theta$ and $\|u_\textsc{e}(x)\|^{~}_{L^2}<\infty$, a singular point may appear as a pole of a meromorphic function.
We denote a denominator polynomial of an irreducible representation of $u(x,\theta)$ as $d(\<v_\theta(x)\>,\theta)$, where $n\in\N$ is the highest power of $e^{i\pi\theta}$ in the denominator polynomial, which is
\begin{align*}
d(x,\theta)=\sum_{p=0,\cdots,n}d_p(x)e^{ip\pi\theta}
%d_0(x)+e^{i\pi\theta}\(d_1(x)+e^{i\pi\theta}\(d_2(x)+e^{i\pi\theta}\(d_3(x)+\cdots+e^{i\pi\theta}
%\(d_{n-1}(x)+e^{i\pi\theta}d_n(x)\)\cdots\)\)\)\!,
\end{align*}
where $d_\bullet(x)$ are real non-singular functions, and .


Since $u(x,1)$ has no-pole owing to the assumption, $d^{ij}_0(x)\neq0$ or $d^{ij}_1(x)\neq0$ at any $x{\in}D(\Delta_\theta)$; thus, singular points of $u(x,\theta)$ exist at $\theta$ yielding $|d(x,\theta)|=0$; this condition fulfils if and only if $[0,1]\ni\theta=0$ or $1$.
However, $u(x,1)$ is finite; thus, the theorem is maintained.

For $\theta\in(-1,1)\setminus\{0\}$, an integrand of $\FTg(f)(\tp)$ has a real exponent concerning $dt:=dx^0$ in $\TsMM$.
We assume the positivity of the energy $E:=\tp_0\geq0$ owing to physics.
Using a complex energy defined as $E_\theta:=Ee^{i\pi\theta}$, (\ref{FL1}) and  (\ref{FL2}) have representations such that: 
\begin{subequations}
\begin{align}
\FTg(f)(\tp)&=\int_0^\infty{e^{iE_\theta t/\hbar}}\hspace{.2em}{f}(t,\vec{\tp})\hspace{.1em}dt
=:\tilde{f}_\mathrm{L}(\tp),\label{LT3}\\
\FTg^{-1}(\tilde{f})(r)&={PV}\int_{\Gamma^{~}_{\hspace{-.1em}E}}{e^{-iE_\theta t/\hbar}}\tilde{f}(E_\theta,\vec{r})
\hspace{.1em}dE,\label{LT4}
\end{align}
with
\begin{align*}
{f}(t,\vec{\tp})&:=\int_\TsMM{e^
{+i{\eta^{~}_\theta}^{\hspace{-.1em}\bcdots}r_\bcdot\tp_\bcdot/\hbar}}f^{~}_\E(x)\hspace{.1em}
dx^1{\wedge}\cdots{\wedge}dx^{n-1},\\
\tilde{f}(E_\theta,\vec{r})&:=\frac{1}{\(2\pi\hbar\)^{n}}\int_\TstMg{e^
{-i{\eta^{~}_\theta}^{\hspace{-.1em}\bcdots}r_\bcdot\tp_\bcdot/\hbar}}\tilde{f}_\mathrm{L}(\tp)\hspace{.1em}
\teee^1\wedge\cdots\wedge\teee^{n-1},
\end{align*}
where  and $dE=d\hp^0$ and $\Gamma^{~}_{\hspace{-.1em}E}$ is an appropriate integration line in a domain of $\tilde{f}(E_\theta,\vec{r})$, where $\vec{\bullet}$ is a three-dimensional space vector.
\end{subequations}

\begin{remark}\textup{(Existence of a Laplace transformation) \cite{zeidler2006quantum}}\\
Suppose there exists some real constant $c$ for the given $E_0\in\R$ such that $|\tilde{f}(E_\theta,r)|\leq c\hspace{.2em}e^{-E_0 t}$ for any $t\geq0$.
Then, the integral \textup{(\ref{LT3})} is a holomorphic function on the half-plane $\{E_\theta\in\C|\textup{Im}[E_\theta]>-\hbar E_0\}$.
We note that $\textup{Im}[E_\theta]=E\sin{(\pi\theta)}>0$ in $\theta\in(0,1)$.

The adjoint transformation \textup{(\ref{LT4})} converges with an arbitrary integration-line parallel to the real axis on the abovementioned half-plain and yields $\FTg^{-1}(\tilde{f})(r)=f^{~}_\E(x)$; thus, it is the inverse Laplace transformation.
\end{remark}

An alternative way to introduce the Fourier transformation geometrically in physics is to utilize symplectic geometry. 
We double the inertial manifold as $\Mg^{symp}:=\Mg\oplus\tMg$ and introduce the Liouville form and the symplectic form such that:
\begin{align*}
\sss&:=\ppp{\wedge}d\rrr\in\Omega^1(\TsMg^{symp})
\intertext{and}
d\sss&:=d\ppp{\wedge}d\rrr\in\Omega^2(\TsMg^{symp}).
\end{align*}
Polarisation is a construction of two $n$-dimensional Hilbert spaces, say  $L^2(\TsMg)$ and $L^2(\TstMg)$, in the $2n$-dimensional space $\Mg^{symp}$\!.
In this case, the Fourier transformation is automorphism in $\Mg^{symp}$ under a restriction owing to polarization.
The inertial manifold is a submanifold of $\Mg^{symp}$, and the global space-time manifold $\MM$ is extended to equip a symplectic structure.
The amphometric tensor is extended to $2n$-dimensional space.
This study does not discuss this method more.


==> settings.tex <==
\makeatletter
\DeclareRobustCommand*\cal{\@fontswitch\relax\mathcal}
\makeatother
\makeatletter
\newcommand*{\rom}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother

\def\slash#1{\not\!#1}
%\def\sr#1{\hspace{-.1em}#1\hspace{-.2em}}
%\def\sro#1{\hspace{-.1em}#1\hspace{-.1em}}

% THEOREM Environments (Examples)----------------------------------------- 
%
\theoremstyle{plain}
\newtheorem{definition}{Definition}
\newtheorem{theorem}[definition]{Theorem}
\newtheorem{lemma}[definition]{Lemma}
\newtheorem{corollary}[definition]{Corollary}
\newtheorem{principle}[definition]{Principle}
\newtheorem{remark}[definition]{Remark}
\newtheorem{fact}[definition]{Fact}
\newtheorem{requirement}[definition]{Requirements}

\theoremstyle{definition}
\newtheorem{example}[definition]{Example}
%
\newcommand{\QED}{\nobreak \ifvmode \relax \else
      \ifdim\lastskip<1.5em \hskip-\lastskip
      \hskip1.5em plus0em minus0.5em \fi \nobreak
      \vrule height0.75em width0.5em depth0.25em\fi}
%
%\newcommand{\bm}[1]{{\mbox{\boldmath $#1$}}}

\def\GLTC{{G\hspace{-.1em}L(2,\C)}}
\def\SLTC{{S\hspace{-.1em}L(2,\C)}}
\def\betaE{{{\bm\eta^{~}_{\textsc{e}}}}}
\def\betaM{{{\bm\eta^{~}_{\textsc{m}}}}}
\def\betaL{{{\bm\eta^{~}_{\textsc{l}}}}}
\def\betaB{{{\bm\eta^{~}_{\bullet}}}}
\def\betathe{{\bm\eta^{~}_\theta}}
\def\betaQ{{\bm\eta^{~}_\theta}}
\def\SOt{{r}}
\def\Ca{{C\hspace{-.1em}aus}}
\def\gB#1{\bm{g}^{~}_{\hspace{-.1em}#1}}
\def\gBa#1{\bm{g}^{a}_{#1}}
\def\gBs#1{\bm{g}_{\hspace{-.1em}#1}}
\def\GLTC{{G\hspace{-.1em}L(2,\C)}}
\def\koko#1{\begin{center}{\color{red}\Large{#1}}\end{center}}
\def\hlf{{1\hspace{-.1em}/\hspace{-.05em}2}}
\def\YMU{Y\hspace{-.15em}M\hspace{-.1em}U\hspace{.2em}}
\def\Rs{{R_{\text{S}}}}

\def\tgamma{\tilde{\gamma^{~}_E}}
\def\ttheta{\tilde{\theta}}
\def\ET{{E,\vartheta}}
\def\tvq{\tilde{\vartheta}}
%
\def\ItN{{\bm{I}_{\SU^{2}}}}
%
\def\Tr{{\mathrm{Tr}\hspace{-.05em}}}
\def\tn{{2\hspace{-.15em}N}}
%
\def\stars{{\star\star}}

\def\bcdot{{\circ}}
\def\bcdots{{\circ\circ}}
\def\bcdott{{\circ\circ\circ\circ}}


\def\bullets{{\bullet\bullet}}

%%%%%%%%%%%%%%%%%%%%%
\def\M{{\cal M}}
\def\MM{\mathscr{M}}
\def\MMM{\mathfrak{M}}

\def\Tm{{T\hspace{-.2em}M}}
\def\Tsm{{T^*\hspace{-.2em}M}}
\def\TM{{T\hspace{-.2em}\M}}
\def\TsM{{T^*\hspace{-.2em}\M}}
\def\TMM{{T\hspace{-.2em}\MM}}
\def\TsMM{{T^*\hspace{-.2em}\MM}}

\def\Mp{{\M_{\hspace{-.1em}p}}}
\def\TMp{{\TM_{\hspace{-.1em}p}}}
\def\TsMp{{\TsM_{\hspace{-.1em}p}}}
\def\Mg{{\M_{\hspace{-.1em}\theta}}}
\def\TMg{{\TM_{\hspace{-.1em}\theta}}}
\def\TsMg{{\TsM_{\hspace{-.1em}\theta}}}

\def\MMg{{\MM_{\hspace{-.1em}\theta}}}
\def\TMMg{{\TMM_{\hspace{-.1em}\theta}}}
\def\TsMMg{{\TsMM_{\hspace{-.1em}\theta}}}

%%%%%%%%%%%%%%%%%%%%

\def\Gso{{{G}_{\hspace{-.2em}S\hspace{-.1em}O}}}
\def\Gsu{{{G}_{\hspace{-.2em}S\hspace{-.1em}U}}}

\def\TsE{{T^*\hspace{-.2em}E}}

\def\GammaSp{{\Gamma_{\hspace{-.1em}\Sp}}}


\def\AA{{\textbf{A}}}
\def\aaa{{\mathfrak a}}
\def\AAA{{\mathfrak A}}
\def\Aa{{\mathscr{A}}}
\def\aa{{\bm{a}}}

\def\bbb{\mathfrak{b}}
\def\BBB{\mathfrak{B}}

\def\OO{{\mathcal O}}
\def\ooo{\mathfrak{o}}
\def\OOO{\mathfrak{O}}
\def\Fym{\mathfrak{ym}}


\def\r{{\bm{r}}}
\def\tbr{\tilde{\r}}

\def\C{\mathbb{C}}
\def\Z{\mathbb{Z}}
\def\K{\mathbb{K}}

\def\QQQ{\mathfrak{Q}}
\def\qqq{\mathfrak{q}}

\def\uuu{\mathfrak{u}}

\def\yyy{\mathfrak{y}}

\def\XXX{\mathfrak{X}}
\def\X{\mathscr{X}}
\def\xxx{\mathfrak{x}}

\def\ZZZ{\mathfrak{Z}}
\def\zzz{\mathfrak{z}}

\def\rp{\hspace{-.1em}\textrm{q}}
\def\p{\bm{p}}
\def\ppp{{\mathfrak p}}
\def\tppp{\tilde{{\mathfrak p}}}
\def\PPP{{\mathfrak P}}

\def\T{\mathscr{T}}
\def\TT{{\mathcal T}}
\def\TTT{{\mathfrak T}}
\def\ttt{{\mathfrak t}}

\def\d{{\cal D}}
\def\D{{\slash{\cal D}}}
\def\Dn{{\nabla}}
\def\FFF{\mathfrak{D}}
\def\td{d_\www}
\def\ddd{\mathfrak{d}}
\def\ds{{\slash{d}}}

\def\v{{\bm{v}}}
\def\V{{\bm{V}}}
\def\vvv{\mathfrak{v}}
\def\VVV{\mathfrak{V}}


\def\u{{\cal{U}}}
\def\UUU{\mathfrak{U}}

\def\FF{{\mathcal F}}
\def\F{{\bm{F}}}
\def\ff{{\cal F}}
\def\fff{\mathfrak{f}}
\def\FFF{\mathfrak{F}}
\def\f{\mathscr{F}}


\def\g{\mathscr{G}}
\def\GGG{\mathfrak{G}}
\def\ggg{\mathfrak{g}}

\def\sss{\mathfrak{s}}
\def\S{{\cal S}}
\def\SSS{{\mathfrak S}}
\def\s{{\mathscr{s}}}
\def\Ss{{\mathscr{S}}}

\def\L{\mathscr{L}}
\def\LL{{\cal L}}
\def\tLL{\tilde{\cal L}}
\def\LLL{{\mathfrak L}}
\def\LD{\pounds}
\def\lll{\mathfrak{l}}

\def\iii{\mathfrak{i}}
\def\ii{{\mathrm I}}

\def\JJJ{{\mathfrak J}}

\def\K{{\mathcal K}}
\def\KK{{\mathscr K}}
\def\KKK{{\mathfrak K}}

\def\H{\mathscr{H}}
\def\HH{{\cal H}}
\def\tHH{\tilde{\cal H}}
\def\hhh{{\mathfrak h}}
\def\HHH{{\mathfrak H}}

\def\B{\mathscr{B}}
\def\BB{\bm{B}}
\def\BBB{{\mathfrak B}}
\def\bbb{{\mathfrak b}}

\def\C{\mathbb{C}}
\def\CCC{{\mathfrak C}}
\def\ccc{{\mathfrak c}}


\def\Epsi{\bm{\mathcal E}}
\def\EEE{\mathfrak{E}}
\def\eee{{\mathfrak e}}

\def\I{\mathscr{I}}
\def\tI{\tilde{\mathscr{I}}}
\def\II{{\cal I}}

\def\NN{\mathscr{N}}
\def\N{\mathbb{N}}


\def\R{\mathbb{R}}
\def\Ri{\mathscr{R}}
%\def\Ri{R}
\def\RRR{\mathfrak{R}}
\def\rrr{\mathfrak{r}}

\def\W{{\cal W}}

%\def\vomega{\varpi}  
\def\vomega{{\mathfrak w}}
\def\www{{\mathfrak w}}
\def\WWW{{\mathfrak W}}
%

%\def\kh{\kappa_\hbar}
\def\kh{\hbar G}

\def\tHHH{\widetilde{\HHH}}
\def\tSSS{\widetilde{\SSS}}
\def\twww{\widetilde{\www}}

\def\sc{{\sss\hspace{-.1em}\ccc}}
\def\MMgr{\M_{\hspace{-.1em}G\hspace{-.1em}R}}
\def\MMvac{\M_{\hspace{-.1em}vac}}
\def\LLvac{\LL_{\hspace{-.1em}vac}}
\def\LLschw{\LL_{\hspace{-.1em}\mathrm{Schw}}}
\def\Thetagr{\Theta_{\hspace{-.1em}vac}}
\def\Evac{{\bm{\E}}_{\hspace{-.1em}vac}}

\def\WWWvac{\WWW_{\hspace{-.1em}vac}}
\def\Mvac{M_{\hspace{-.1em}vac}}
\def\WWWgr{\WWW_{\hspace{-.1em}G\hspace{-.1em}R}}
\def\Mgr{M_{\hspace{-.1em}G\hspace{-.1em}R}}
\def\sssvac{\sss_{\hspace{-.1em}vac}}
\def\sssgr{\sss_{\hspace{-.1em}G\hspace{-.1em}R}}
\def\Sgr{S_{\hspace{-.1em}G\hspace{-.1em}R}}

\def\sc{{\sss\hspace{-.1em}\ccc}}
\def\scgr{\sss\hspace{-.1em}\ccc_{\hspace{-.1em}G\hspace{-.1em}R}}
\def\scvac{\sss\hspace{-.1em}\ccc_{\hspace{-.1em}vac}}
\def\sc{{\sss\hspace{-.1em}\ccc}}

\def\Pivac{{\Pi_{\hspace{-.1em}vac}}}

\def\={{\hspace{-.1em}=\hspace{-.1em}}}

\def\LLambda{\bm{\Lambda}}

\def\SO{{\hspace{-.1em}S\hspace{-.1em}O\hspace{-.1em}}}
\def\SU{{\hspace{-.1em}S\hspace{-.1em}U\hspace{-.1em}}}
\def\Uo{{\hspace{-.1em}U\hspace{-.2em}_\textit{1}\hspace{-.1em}}}
\def\Sp{{\hspace{-.1em}s\hspace{-.1em}p\hspace{.1em}}}
\def\SG{{\hspace{-.2em}s\hspace{-.1em}g}}
\def\hSG{{\hspace{-.2em}\widehat{s\hspace{-.1em}g}}}
\def\EM{{\hspace{-.1em}E\hspace{-.1em}M\hspace{-.1em}}}
\def\ch{{\hspace{-.1em}c\hspace{-.1em}h}}
\def\SUO{{\SU\hspace{-.1em}\otimes\SO}}

%\def\Cl{{\textoesch{Cl}\hspace{.1em}}}
\def\Cl{{\mathcal C\hspace{-.1em}l}}

\def\Slash#1{{\not\!#1}}
%\def\Slash#1{{\hspace{-.2em}\slash#1\hspace{.2em}}}
\def\slashD{{D\hspace{-.7em}\slash\hspace{.5em}}}
\def\sss{{\mathfrak s}}
\def\uuu{{\mathfrak u}}

\def\wcs{{\www\hspace{-.1em}\cdot\hspace{-.1em}\Ss}}
\def\wcss{{\(\iota_{{\gamma^{~}_E}_\Sp}\www\)
\hspace{-.1em}\cdot\hspace{-.1em}S}}

\def\gasu{{\(\iota_{{\gamma^{~}_E}_\Sp}\AAA^{~}_\SU\)}}

\def\cP{{\hspace{-.1em}c\hspace{-.05em}\mathrm{P}}}
\def\Poin{{\hspace{-.1em}\mathrm{P}}}
\def\cov{{\hspace{-.1em}cov}}

\def\hpi{{\hat\tau}}
\def\hPi{{\hat\Tau}}

\def\YM{{\mathrm{YM}}}
\def\MYM{{\mathrm{MYM}}}
\def\ym{{\textrm{Y}\hspace{-.1em}\textrm{M}}}

\def\Dc{{\hspace{-.1em}\textrm{D}c}}
\def\hSU{{\widehat\SU}}
\def\cG{{c^{~}_{\hspace{-.1em}g\hspace{-.1em}r}}}
\def\bcG{{\bm{c}^{~}_{\hspace{-.1em}g\hspace{-.1em}r}}}
\def\cGz{{c^{~}_{\hspace{-.1em}g\hspace{-.1em}r}}}
\def\cGo{{{c}^{~}_{\hspace{-.1em}g\hspace{-.1em}r}}}
\def\hcG{{{c}^{~}_{\hspace{-.1em}g\hspace{-.1em}r}}}
\def\DSp{{\D^{~}_{\hspace{-.1em}\Sp}}}
\def\dSp{{\slash{d}^{~}_{\hspace{-.1em}\Sp}}}
\def\dSg{{\slash{d}^{~}_{\SG}}}
\def\dSgp{{\slash{d}^{+}_{\SG}}}
\def\dSgm{{\slash{d}^{-}_{\SG}}}
\def\dSgpm{{\slash{d}^{\pm}_{\SG}}}
\def\hdSg{{\slash{\hat{d}}^{~}_{\SG}}}
\def\DSpE{{\D_{\hspace{-.1em}\Sp}^E}}


\def\dR{{de\hspace{.1em}Rham }}

\def\cs{{\ccc\hspace{-.1em}\sss}}
\def\SM{{\hspace{-.1em}\setminus\hspace{-.1em}}}

\def\gdg{\bm{g}^{-1}_\SU\hspace{.1em}d\bm{g}_\SU^{~}}

\def\HD{{\widehat{\mathrm{H}}}}
\def\HDi{{\widehat{\mathrm{H}}^{-1}}}
\def\TxT{{2\hspace{-.1em}\times\hspace{-.1em}2}}

\def\sigmav{{{\sigma^{~}_{\hspace{-.1em}v}}}}
\def\sigmag{{{\sigma^{~}_{\hspace{-.1em}g}}}}
\def\tsigmag{{{\tilde\sigma^{~}_{\hspace{-.1em}g}}}}
\def\sigmaeta{{{\sigma^{~}_{\hspace{-.1em}\eta}}}}
\def\sigmath{{{\sigma^{~}_{\hspace{-.1em}\theta}}}}
\def\tsigmath{{{\tilde\sigma^{~}_{\hspace{-.1em}\theta}}}}
\def\sigmaet{{\sigma_{\hspace{-.1em}\eta_\theta}}}

\def\KP{{K\hspace{-.2em}P}}
\def\dr{{\textrm{d\hspace{-.1em}R}}}
\def\theEp{{\theta_\varepsilon}}



%\def\cod{{\rotatebox[origin=c]{180}{$\delta$}}}
\def\cod{{\bar{d}}}
%\def\cod{{\hspace{.1em}\reflectbox{\textit{d}}\hspace{-.1em}}}
%\def\cod{{\delta}}

\def\<{{\langle}}
\def\>{{\rangle}}

\def\norm{{\textit{norm}}}

\def\Land{{~\land~}}
\def\Lor{{~\lor~}}


\def\({\left(}
\def\){\right)}

\def\tMg{{\tilde{\M}_{\hspace{-.1em}\theta}}}
\def\TtMg{{{T\hspace{-.2em}\tilde{\M}}_{\hspace{-.1em}\theta}}}
\def\TstMg{{{T^*\hspace{-.2em}\tilde{\M}}_{\hspace{-.1em}\theta}}}
\def\TtM{{{T\hspace{-.2em}\tilde{\M}}}}
\def\TstM{{{T^*\hspace{-.2em}\tilde{\M}}}}

\def\teee{\tilde{\mathfrak{e}}}
%\def\teee{d\hp}
%\def\teee{\ppp}
%\def\teee{\xxx}
\def\trrr{\tilde{\rrr}}
\def\heee{d\hr}
\def\teepp{\tilde{\mathfrak{e}}_\mathfrak{p}}

\def\CMm{{C\hspace{-.15em}M}}
\def\CM{{C\hspace{-.15em}\tilde{M}}}
\def\MC{{\tilde{M}\hspace{-.15em}C}}
%\def\pF{{p\hspace{-.1em}F}}
\def\pF{{F\hspace{-.1em}T}}
\def\FT{{C\hspace{-.2em}F}}

\def\FTg{{C\hspace{-.2em}F_\theta}}
\def\CMmg{{C\hspace{-.15em}M_\theta}}
\def\CMg{{C\hspace{-.15em}\tilde{M}_\theta}}
\def\MCg{{\tilde{M}\hspace{-.15em}C_\theta}}

\def\tp{\tilde{p}}
\def\tx{\tilde{\xi}}
\def\tr{\tilde{r}}

\def\hp{\hat{p}}
\def\hx{\hat{\xi}}
\def\hr{\hat{r}}

\def\bp{\bm{p}}
\def\vp{\vec{p}}
\def\bq{\bm{q}}
\def\bx{\bm{x}}
\def\bxi{\bm{\xi}}
\def\br{\bm{r}}
\def\vr{\vec{r}}

\def\btp{\tilde{\bp}}
\def\vtp{\vec{\tilde{p}}}
\def\btx{\tilde{\bx}}
\def\btxi{\tilde{\bxi}}
\def\btr{\tilde{\br}}

\def\vvvp{{\VVV\hspace{-.1em}_\mathrm{p}\hspace{-.15em}}}
\def\tvvv{{\tilde\vvv}}
\def\tvvvp{{\tvvv\hspace{-.1em}_\mathrm{p}}}

\def\deteps{{\mathrm{det}\left[\E\right]}}
\def\deteta{{\mathrm{det}\left[\bm{\eta}^{~}_\theta\right]}}

\def\fdl{{\bm{[}}}
\def\fdr{{\bm{]}}}

\def\E{{\mathcal E}}

\def\fsch{f_{\textrm{S}}}
\def\sinvt{\sin{\hspace{-.15em}\vartheta}}
\def\sintvt{\sin^2{\hspace{-.15em}\vartheta}}

\def\gm2{{g_\mu\hspace{-.2em}-\hspace{-.1em}2}}

\def\pb{{\bar{p}}}

